Instantaneous Relaying: Optimal Strategies and Interference Neutralization

In a multi-user wireless network equipped with multiple relay nodes, some relays are more intelligent than other relay nodes. The intelligent relays are able to gather channel state information, perform linear processing and forward signals whereas the dumb relays is only able to serve as amplifiers. As the dumb relays are oblivious to the source and destination nodes, the wireless network can be modeled as a relay network with *smart instantaneous relay* only: the signals of source-destination arrive at the same time as source-relay-destination. Recently, instantaneous relaying is shown to improve the degrees-of-freedom of the network as compared to classical cut-set bound. In this paper, we study an achievable rate region and its boundary of the instantaneous interference relay channel in the scenario of (a) uninformed non-cooperative source-destination nodes (source and destination nodes are not aware of the existence of the relay and are non-cooperative) and (b) informed and cooperative source-destination nodes. Further, we examine the performance of interference neutralization: a relay strategy which is able to cancel interference signals at each destination node in the air. We observe that interference neutralization, although promise to achieve desired degrees-of-freedom, may not be feasible if relay has limited power. Simulation results show that the optimal relay strategies improve the achievable rate region and provide better user-fairness in both uninformed non-cooperative and informed cooperative scenarios.

==> tikz_ach_reg1.tex <==
\begin{tikzpicture}
\pgfplotsset{every axis legend/.append style={
at={(0.5,1.03)},
anchor=south}}
\begin{axis}[legend columns=1, xlabel={$R_1$ (bits/sec/Hz)}, ylabel={$R_2$ (bits/sec/Hz)}]
\addplot coordinates {(2.68,0) (2.6800,4.5432) (0,4.5432) };
\addplot coordinates {(3.2584,0) (2.8009,0.7041) (2.8009 ,1.1935) (2.8009, 1.6733) (2.7476,2.2914) (2.7269,2.8389) (2.7159,3.3523) (2.7044, 3.9121) (2.6965, 4.4613) (0,4.8094)};
\legend{a,b};
\end{axis}
\end{tikzpicture}

